Efficient Decentralized Deep Learning by Dynamic Model Averaging

We propose an efficient protocol for decentralized training of deep neural networks from distributed data sources. The proposed protocol allows to handle different phases of model training equally well and to quickly adapt to concept drifts. This leads to a reduction of communication by an order of magnitude compared to periodically communicating state-of-the-art approaches. Moreover, we derive a communication bound that scales well with the hardness of the serialized learning problem. The reduction in communication comes at almost no cost, as the predictive performance remains virtually unchanged. Indeed, the proposed protocol retains loss bounds of periodically averaging schemes. An extensive empirical evaluation validates major improvement of the trade-off between model performance and communication which could be beneficial for numerous decentralized learning applications, such as autonomous driving, or voice recognition and image classification on mobile phones.

==> sec_theory_prop3.tex <==
\section{Extended Proof of Proposition 3}
\label{sec:theory}
Given an online learning algorithm $\onlineAlgo$, the \defemph{periodic averaging protocol} $\periodProt=(\onlineAlgo,\syncop_b)$ synchronizes the current model configuration ${\modelconf}$ every $b\in\N$ time steps by replacing all local models by their joint average
$
\avgmodel=\sfrac{1}{\totalLearners}\sum_{\learner=1}^{\totalLearners}\model^\learner
$. That is, the synchronization operator is given by
\[
\syncop_b(\modelconf_t)=	\begin{cases}
\left(\avgmodel_\round,\dots,\avgmodel_\round\right), &\text{ if } b \equiv O(\round)\\%\mid \round\\
\enspace\modelconf_\round = (\model_\round^1,\dots,\model_\round^\totalLearners), &\text{ otherwise}\\
\end{cases}\enspace .
\]
A special case of this is the \defemph{continuous averaging protocol} $\contProt=(\onlineAlgo,\syncop_1)$ that synchronizes every round, i.e., $
\syncop_1\left(\modelconf\right)=\left(\avgmodel,\dots,\avgmodel\right)
$.
As base learning algorithm we use mini-batch SGD algorithm $\uprule^{MB}_{B,\eta}$~\citep{dekel/jmlr/2012} which is commonly used in deep learning~\citep{bottou1991stochastic}. One step of this learning algorithm given the model $\model\in\modelSpace$ can be expressed as
\[
\uprule^{MB}_{B,\eta}(\model) = \model -\eta\sum_{j=1}^B \nabla\loss^j(\model)\enspace .
\]
For this, let $\contProt^{MB}=(\uprule^{MB}_{B,\eta},\syncop_1)$ denote the continuous averaging protocol using mini-batch SGD. Then for $\totalLearners\in\N$ learners, mini-batch size $B\in\N$, $\totalLearners B$ training samples $(\sample_1,\truelabel_1),\dots,(\sample_{\totalLearners B},\truelabel_{\totalLearners B})$, corresponding loss functions $\loss^\learner(\cdot) = \loss(\cdot,\sample_\learner,\truelabel_\learner)$, a learning rate $\eta\in\R_+$, and a model configuration $\modelconf=(\model,\dots,\model)$, one step of $\contProt^{MB}$ can be expressed as
\[
\syncop_1\left(\left(\uprule^{MB}_{B,\eta}(\model),\dots,\uprule^{MB}_{B,\eta}(\model)\right)\right) = \frac{1}{\totalLearners}\sum_{\learner=1}^{\totalLearners}\left(\model - \eta\textstyle\sum_{j=1}^{B}\nabla\loss^{(\learner - 1)B + j}(\model)\right)\enspace .
\]
We compare $\contProt^{MB}$ to the serial application of mini-batch SGD. 
%
%Let $\uprule^{SGD}$ denote the stochastic gradient descent learning algorithm and $\contProt^{SGD}=(\uprule^{SGD},\syncop_1)$ the continuous averaging protocol with SGD. Then for $\totalLearners\in\N$ training examples $(\sample_1,\truelabel_1),\dots,(\sample_{\totalLearners},\truelabel_\totalLearners)$, corresponding loss functions $\loss^\learner(\cdot) = \loss(\cdot,\sample_\learner,\truelabel_\learner)$, a learning rate $\eta\in\R_+$, and a model configuration $\modelconf=(\model,\dots,\model)$, one step of $\contProt^{SGD}$ can be expressed as
%\[
%\syncop_1\left(\left(\uprule^{SGD}_{\eta}(\model),\dots,\uprule^{SGD}_{\eta}(\model)\right)\right) = \frac{1}{\totalLearners}\sum_{\learner=1}^{\totalLearners}\left(\model - \eta\nabla\loss^\learner(\model)\right)\enspace .
%\]
It can be observed straight-forwardly that continuous averaging with mini-batch SGD on $\totalLearners\in\N$ learners with mini-batch size $B$ is equivalent to serial mini-batch SGD with a mini-batch size of $\totalLearners B$ and a learning rate that is $\totalLearners$ times smaller.

\noindent
\textcolor{red}{(Reviewer \#1 argues that in one round, serial mini-batch would have processed $m$ mini-batches which indeed would lead to different results, as he pointed out. However, as stated here and again in the proposition, serial mini-batch uses a batch size of $mB$, thus in one round it performs only one update. Therefore, the gradients of the loss function are the same for all samples in one round.)}
\begin{pr}
For $\totalLearners\in\N$ learners, a mini-batch size $B\in\N$, $\totalLearners B$ training samples $(\sample_1,\truelabel_1),\dots,(\sample_{\totalLearners B},\truelabel_{\totalLearners B})$, corresponding loss functions $\loss^\learner(\cdot) = \loss(\cdot,\sample_\learner,\truelabel_\learner)$, a learning rate $\eta\in\R_+$, and a model $\model\in\modelSpace$, it holds that
\[
\syncop_1\left(\left(\uprule^{MB}_{B,\eta}(\model),\dots,\uprule^{MB}_{B,\eta}(\model)\right)\right) = \uprule^{MB}_{\totalLearners B,\sfrac{\eta}{\totalLearners}}(\model)\enspace .
\]
\textcolor{darkred}{That is, averaging $m$ models, each of which processed one one mini-batch of $B$ examples, is equivalent to serial mini-batch SGD with a batch size of $mB$.}
\label{prop:contAvgEqualMiniBatch}
\end{pr}
\begin{proof}
For a model $\model \in \modelSpace$ it holds that
\begin{equation}
\begin{split}
\syncop_1&\left(\left(\uprule^{MB}_{B,\eta}(\model),\dots,\uprule^{MB}_{B,\eta}(\model)\right)\right) = \frac{1}{\totalLearners}\sum_{\learner=1}^{\totalLearners}\left(\model - \eta\sum_{j=1}^{B}\nabla\loss^{(\learner - 1)B + j}(\model)\right)\\
&= \frac{1}{\totalLearners}\totalLearners \model - \frac{1}{m}\eta\sum_{\learner=1}^{\totalLearners}\sum_{j=1}^{B}\nabla\loss^{(\learner - 1)B + j}(\model)\\
&= \model  - \frac{1}{m}\eta\sum_{j=1}^{\totalLearners B}\nabla\loss^{j}(\model)=\uprule^{MB}_{\totalLearners B,\sfrac{\eta}{\totalLearners}}(\model)\enspace .
\end{split}
\label{eq:proposition3}
\end{equation}
%\textcolor{darkred}{Let $\model_{\round+1}^\text{cont} = \syncop_1\left(\left(\uprule^{MB}_{B,\eta}(\model_\round),\dots,\uprule^{MB}_{B,\eta}(\model_\round)\right)\right)$ be the model maintained by continuous averaging $\contProt^{MB}$ and $\model_{\round+1}^\text{serial} = \uprule^{MB}_{\totalLearners B,\sfrac{\eta}{\totalLearners}}(\model_\round)$ be the model maintained by serial mini-batch SGD $\uprule^{MB}_{\totalLearners B,\sfrac{\eta}{\totalLearners}}$. Given that both models are equally initialized, i.e., $\model_{0}^\text{cont} = \model_{0}^\text{serial}$, then it follows from Equation~\ref{eq:proposition3} that for all $\round\in\N$ it holds that $\model_{\round}^\text{cont} = \model_{\round}^\text{serial}$. That is, continuous averaging with $m$ learners, using mini-batch SGD with batch size $B$ and a learning rate of $\eta$ is equivalent to serial mini-batch SGD with batch size $mB$ and learning rate $\sfrac{\eta}{m}$.}
%
%}
%\substack{\\ \text{this equality.}}
%\begin{equation*}
%\begin{split}
%\syncop_1&\left(\left(\uprule^{SGD}_{\eta}(\model),\dots,\uprule^{SGD}_{\eta}(\model)\right)\right) = \frac{1}{\totalLearners}\sum_{\learner=1}^{\totalLearners}\left(\model - \eta\nabla\loss^\learner(\model)\right)\\
%&= \frac{1}{\totalLearners}\totalLearners \model - \frac{1}{m}\eta\sum_{\learner=1}^{\totalLearners}\nabla\loss^\learner(\model)
%= \model - \frac{1}{m}\eta\sum_{\learner=1}^{\totalLearners}\nabla\loss^\learner(\model) = \uprule^{MB}_{\totalLearners,\sfrac{1}{\totalLearners}}\enspace .
%\end{split}
%\end{equation*}
\qed
\end{proof}
In particular, Proposition~\ref{prop:contAvgEqualMiniBatch} holds for continuous averaging with a mini-batch size of $B=1$, i.e., classic stochastic gradient descent. 

\vspace{10cm}
\pagebreak

From Proposition~\ref{prop:contAvgEqualMiniBatch} follows that continuous averaging is consistent as in Definition~\ref{def:efficiency}, since it retains the loss bound of serial mini-batch SGD and classic SGD. Theorem~4 in~\citet{kamp2016kernels} proves that for SGD, dynamic averaging has a predictive performance similar to any periodically communicating protocol, in particular to $\syncop_1$.
Thus it follows that dynamic averaging using stochastic gradient descent for training deep neural networks is consistent.
Theorem~2 in~\citet{kampAdaptive2014} shows that the communication of the dynamic averaging protocol using stochastic gradient descent and a divergence threshold $\Delta$ is bounded by
\[
\cummcomm{}{\totalRounds,\totalLearners}\in\bigO{\frac{\commcost{}(\modelconf)}{\sqrt{\Delta}}\cummloss{}{\totalRounds,\totalLearners}}\enspace ,
\]
where $\commcost{}(\modelconf_{\round})$ is the number of bytes required to be communicated to average a set of deep neural networks. Since each neural network has a fixed number of weights, this cost is in $\bigO{\totalLearners}$. It follows that dynamic averaging is adaptive.
Thus using dynamic averaging with stochastic gradient descent for the decentralized training of deep neural networks is efficient as in Definition~\ref{def:efficiency}.

Note that the synchronization operator can be implemented using different assumptions on the system's topology and communication protocol, i.e., in a peer-to-peer fashion, or in a hierarchical communication scheme. For simplicity, in our analysis of the communication of different synchronization operators we assume that the synchronization operation is performed by a dedicated coordinator node. This coordinator is able to poll local models, aggregate them and send the global model to the local learners. 
